First Passage Percolation with Queried Hints

Solving optimization problems leads to elegant and practical solutions in a wide variety of real-world applications. In many of those real-world applications, some of the information required to specify the relevant optimization problem is noisy, uncertain, and expensive to obtain. In this work, we study how much of that information needs to be queried in order to obtain an approximately optimal solution to the relevant problem. In particular, we focus on the shortest path problem in graphs with dynamic edge costs. We adopt the $\textit{first passage percolation}$ model from probability theory wherein a graph $G'$ is derived from a weighted base graph $G$ by multiplying each edge weight by an independently chosen random number in $[1, \rho]$. Mathematicians have studied this model extensively when $G$ is a $d$-dimensional grid graph, but the behavior of shortest paths in this model is still poorly understood in general graphs. We make progress in this direction for a class of graphs that resemble real-world road networks. Specifically, we prove that if $G$ has a constant continuous doubling dimension, then for a given $s-t$ pair, we only need to probe the weights on $((\rho \log n )/ \epsilon)^{O(1)}$ edges in $G'$ in order to obtain a $(1 + \epsilon)$-approximation to the $s-t$ distance in $G'$. We also generalize the result to a correlated setting and demonstrate experimentally that probing improves accuracy in estimating $s-t$ distances.

==> checklist.tex <==
\section*{Checklist}


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No] We do not provide the code for our experiments, but do provide the data used (OSM graph files) and the paper includes a complete description of the experiment.
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes] We do not provide the code that we used in our experiments. However, we do provide the Washington and Baden-Wurttemberg graph files and our paper includes a complete description of the algorithm used to run the experiment (Algorithm \ref{alg:demand_alg}), so our experiments are reproducible.
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable] Our experiments do not include a training process.
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable] Our experiments only compare results. Runtime is irrelevant, so the machine used is also irrelevant.
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Yes]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable] There is no new assets released or curated.
   \item Information about consent from data providers/curators. [Yes]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

\end{enumerate}

==> demands.tex <==
\section{Correlated Model: Independent Demands}
In this section, we consider a ``independent demands'' model, where we allow correlations in the edge weight distribution. Suppose that there are $m$ hidden variables $y=(y_1, y_2, \ldots, y_m)$. Each hidden variable $y_i$ follows an independent distribution $\mathcal{D}_i$ within the range $[\lambda_i, \lambda_i \cdot \rho]$. Each edge $e\in E$ has actual weight in the following form:
\begin{equation} \label{eqn:demand_constraint}
   w_e' = \left(\sum_{i=1}^{m} \lambda_{i}^e \cdot y_i\right)^\beta \cdot w_e, 
\end{equation}
where $\{\lambda_i^e\}_{i \in [m], e \in E}$ are known non-negative real numbers, called \emph{dependence parameters}. These parameters indicates the influence of hidden variable $y_i$ on the edge $e$. To interpret this model, we can view the hidden variables $\{y_i\}$ as some major demand types of users. Each type of demand will affect a subset of edges and create certain amount of traffic (or flow) on these edges. The demand amount of type $i$ is denoted by $y_i$. Each edge has total traffic as a linear combination (i.e. $\sum_{i=1}^{m} \lambda_{i}^e \cdot y_i$) of the all the demands that affect it. $f(t)=t^\beta$ is a power function mapping the total traffic on an edge to its traversing time, where $\beta$ is generally set to $4$ in the literature [cite?].

Instead of probing on edges, in this model we are allowed to probe on the demands (i.e. $y_i$'s).

For each hidden variable $y_i$, define cluster $i$ as $C_i = \{e: \lambda_i^e > 0\}$, i.e. the set of edges that are actually influenced by $y_i$. In this model, we apply the same idea as \cref{alg:main_alg} to probe the demands with the largest cluster sizes, after a normalization step. The algorithm is as follows: [Some intuitions and analysis here..]

\begin{algorithm}[ht]
\caption{}
\label{alg:demand_alg}
%\algrenewcommand{\Procedure}[2]{\textbf{procedure}\ \textsc{#1}\left(#2\right)}
\begin{algorithmic}
    \Procedure{ProbingDemands}{$s, t, G, \{\mathcal{D}_i\}_{i \in [m]}, \{\lambda_i\}_{i\in [m]}, \{\lambda_i^e\}_{i \in [m], e \in E}, y$}
        \For{\( i \in [m], e \in E \)}
            % \State \( \tilde{\lambda}_{i}^e \gets \frac{\lambda_i \cdot \lambda_i^e}{\sum_{j \in [m]} \left(\lambda_j^e \cdot \lambda_j \right)}; \) 
            \State \( \tilde{w}_e \gets w_e \cdot \left(\sum_{i \in [m]} \left( \lambda_i^e \cdot \lambda_i \right) \right)^\beta; \) 
        \EndFor
        \State \( \tilde{G} \gets (V, E, \tilde{w});\ L \gets d_{\tilde{G}}(s,t); \) \Comment{Compute the edge weights under basic demands}
        \State \( H \gets \tilde{G}[\tilde{G} \cap B^{\tilde{G}}_{s}(\rho^\beta \cdot L)]; \)
        \For{\( i \in [m] \)}
            \State \( \Omega_i \gets \sum_{e\in E_H \cap C_i} \tilde{w}_e; \) \Comment{Compute the effective cluster size of demand $y_i$}
            \If {\( \Omega_i > \frac{\eps^2\cdot L}{16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell} \)}
                \State \( y'_i \gets y_i; \) \Comment{Probe on $y_i$ if the effective size is large}
            \Else
                \State \( y'_i \sim \mathcal{D}_i;\) \Comment{Sample from $\mathcal{D}_i$ otherwise}
            \EndIf
        \EndFor
        \For{\( e \in E_H \)}
            \State \( w_e^H \gets\left(\sum_{i=1}^{m} \lambda_{i}^e \cdot y_i'\right)^\beta \cdot w_e; \)
        \EndFor        
        \State \Return \( d_H(s,t). \)
    \EndProcedure
\end{algorithmic}
\end{algorithm}

We have the following theorem which bounds the number of demand probes in order to estimate the shortest path length:
\begin{restatable}[]{theorem}{thmHighwayDemandsAssumption}
    \label{thm:highway-demands}
    Given a weighted graph $G = (V, E, w)$. Suppose there are some hidden random variables $\{y_i\}_{i \in [m]}$, each follows an independent bounded distribution within the range $[\lambda_i,\ \rho \cdot \lambda_i]$. Suppose that $G$ satisfies the following:
    \begin{itemize}
        \item [1.] $G$ has continuous highway dimension $h$ under basic demands;
        \item [2.] Every $C_i$ represents a shortest path under basic demands;
        \item [3.] Every edge in $G$ only falls in at most $\ell$ different clusters; 
    \end{itemize}
    And in the actual graph $G' = (V, E, w')$, $w'$ satisfies \cref{eqn:demand_constraint} with dependence parameters $\{\lambda_i^e\}_{i \in [m], e \in E}$.
    Then, \cref{alg:demand_alg} uses at most
    $\left(\frac{\log n\cdot \rho^{\beta} \cdot \ell}{\eps^2}\right)^{O(\log h)}$ probes on the demands and returns a $(1+\epsilon)$-approximate shortest path in $G'$ with high probability.
\end{restatable}

We define the \emph{normalized size} of a cluster $C_i$ as its actual size under the basic demand, that is $\sum_{e\in C_i} \tilde{w}_e$ in \cref{alg:demand_alg}. In order to prove the above theorem, we first present a lemma where we show that a ball cannot intersect with too many clusters with large normalized cluster sizes. A cluster $C_i$ is called $\Gamma$-effectively large if its normalized size is at least $\Gamma$.  

\begin{lemma} \label{lem:cluster_bounded}
    In $\tilde{G}$, any $R$-radius ball centered at a point $s$ in the graph intersects with $h^2 \cdot \left( \frac{R}{\Gamma} \right)^{\log h}$ $\Gamma$-effectively large clusters.
\end{lemma}
\begin{proof}
    % We first prove that an $r$-radius ball can only intersect with $h\cdot \ell$ different clusters with total weight in the range $(r,\ 3r]$. By the definition of the highway dimension, we have each cluster as the shortest path inside the $4R$-radius ball contains at least one of the highway points. By the third property, we know that each highway point is covered by at most $\ell$ different clusters. Therefore, the $R$ radius ball will intersect with at most $h\cdot \ell$ clusters with normalized size in the range $(r,\ 3r]$. 

    % We classify the normalized sizes of the clusters into buckets: $$(\Gamma, 3\Gamma], (3\Gamma, 9\Gamma], \ldots, (3^{\lfloor \log (2R / \Gamma) \rfloor} \cdot \Gamma, 3^{\lfloor \log (2R / \Gamma) \rfloor + 1} \cdot \Gamma].$$

    % If we view the clusters normalized size larger than $2R$ as its intersecting part with the $R$-radius ball (so its size is at most $2R$ as the intersection is still a shortest path), all the $\Gamma$-large clusters can be put into one of the buckets according to its size range. 

    % Since we can cover the $R$-radius ball with $h^{\lceil \log R/r \rceil}$ $r$-radius balls, the total number of $\Gamma$-effectively large clusters intersecting with the $R$-radius ball is at bounded by 
    % \begin{align*}
    %     \sum_{k = 0}^{\lfloor \log (2R / \Gamma) \rfloor} h\cdot \ell \cdot h^{\left\lceil \log \left( \frac{R}{3 ^ {k} \cdot \Gamma} \right) \right\rceil} &\le h\cdot \ell \cdot (h ^{ \lceil\log \frac{R}{\Gamma}\rceil})\cdot \frac{h}{h - 1}\\
    %     &\le h\cdot \ell \cdot \left(\frac{R}{\Gamma}\right)^{ \log h} \cdot \frac{h^2}{h - 1}\\
    %     & = O\left(\ell \cdot h^3 \cdot \left(R/\Gamma\right)^{\log h} \right). 
    % \end{align*}
    We first prove that an $r$-radius ball can only intersect with $h\cdot \ell$ different clusters with total weight in the range $(r,\ \infty)$. If a path is intersecting the $r$-radius ball and has total length larger than $r$, it must contain a subset of edges with normalized size greater than $r$ that form a shortest path inside the $4r$-radius ball centered at $s$. By the definition of the highway dimension, we the shortest path inside the $4r$-radius ball contains at least one of the highway points. By the third property, we know that each highway point is covered by at most $\ell$ different clusters. Therefore, the $r$ radius ball will intersect with at most $h\cdot \ell$ clusters with normalized size in the range $(r,\ \infty)$. 
 
    Since the continuous doubling dimension of $G$ is bounded by $\log h$, we can cover the $R$-radius ball with $h^{\lceil \log R/r \rceil}$ $r$-radius balls. Let $r = \Gamma$. Each $r$-radius ball intersects with at most $h\cdot \ell$ $\Gamma$-effectively large clusters, the total number of $\Gamma$-effectively large clusters intersecting with the $R$-radius ball is at bounded by $h^{\lceil \log R/\Gamma \rceil} \cdot h \cdot \ell \le h^2 \cdot \left( \frac{R}{\Gamma} \right)^{\log h}$. 
\end{proof}
After the normalization step each edge in $\tilde{G}$ only varies within a multiplicative factor of $\rho^{\beta}$, we extract the subgraph with all the candidate shortest paths and denote it by $H$ in the algorithm. Since any shortest path has original length at most $\rho^\beta \cdot L$. $H$ has radius at most $\rho^\beta \cdot L$. Recall the definition of $\Omega_i$ in \cref{alg:demand_alg} and the construction of $y'$ as a combination of probed $y_i$'s (whose normalized sizes are larger than $\Gamma'$) and some fake samples, we have the following lemma:
\begin{lemma} \label{lem:concentrate}
    If all unprobed demands $y_i$ satisfies $$\Omega_i \le \frac{\eps^2\cdot L}{16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell}, $$ then the shortest path $\delta$, as a function of fake hidden variables $y'$, satisfies $$\Pr\bigg[\big|\delta(y') - \mathbb{M} \, \delta \big| > \frac{\eps \cdot L}{2} \bigg] \le \frac{1}{2n},$$ where $\mathbb{M}$ is the median of $\delta$ on the distribution of all unprobed demands. 
\end{lemma}
\begin{proof}
    Assume the shortest path is a subset of edges and is a function $p(y)$ of the hidden variables $y$. Define $\alpha_i(y) = \sum_{j \in p(y)\cap H \cap C_i} (\rho^\beta - 1) \cdot {\tilde{w}_j}$. Denote $\delta(y)$ the shortest path length function of the hidden variables $y$. Consider two set of hidden variables $y_1$ and $y_2$. When the hidden variables are $y_1$, the shortest path is denoted by $p(y_1)$. If we continue using the path $p(y_1)$ when the actual hidden variables are $y_2$, the length of $p(y_1)$ is bounded by $\delta(y_1) + \sum_{i: y_1^{(i)} \neq y_2^{(i)}} \alpha_i (y_1)$. Since the actual shortest path length when the hidden variables are $y_2$ is at most the length of $p(y_1)$, we have $\delta(y_2) \le \delta(y_1) + \sum_{i: y_1^{(i)} \neq y_2^{(i)}} \alpha_i (y_1)$.

    Let $|\alpha(y)|^2 = \sum_{i} \alpha_i(y)^2$. Since we have 
    \begin{align*}
        \sum_i \alpha_i(y) &= \sum_i \left( \sum_{j \in p(y)\cap H \cap C_i} \tilde{w}_j \cdot (\rho^\beta - 1) \right)\\
        &\le \sum_i \left( \sum_{j \in p(y)\cap H \cap C_i} \tilde{w}_j \cdot \rho^\beta  \right)\\
        &\le \sum_{j \in p(y)\cap H} \ell \cdot \tilde{w}_j \cdot \rho^\beta \tag{By Property 3 of \cref{thm:highway-demands}}\\
        &\le \ell\cdot L\cdot \rho^{2\beta}. \tag{Since $\sum_{j\in p(y)} \tilde{w}_j \le L \cdot \rho^\beta$}
    \end{align*}
 
   Let $\Gamma' = \frac{\eps^2\cdot L}{16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell}$. Since $\forall i$, $\alpha_i(y) \le \rho^\beta \cdot \Omega_i \le \rho^\beta \cdot \Gamma'$, we have $$\sup_{y}|\alpha(y)|^2 \le \sup_y \left\{\left(\max_i \alpha_i(y) \right) \cdot \sum_{i} \alpha_i(y) \right\}\le \ell \cdot L \cdot \rho^{3\beta}\cdot \Gamma'.$$

    By applying Talagrand's Inequality with $\sup_{y} |\alpha(y)|^2 \le \ell \cdot L \cdot \rho^{3\beta}\cdot \Gamma'$, we have: $$\Pr\bigg[\big|\delta(y') - \mathbb{M} \, \delta \big| > \frac{\eps \cdot L}{2} \bigg] \le \exp\left[\frac{-\eps^2\cdot L^2}{16\sup_{y\in Y}|\alpha(y)|^2}\right] \le \exp\left[\frac{-\eps^2\cdot L}{16 \ell \cdot \rho^{3\beta}\cdot \Gamma'}\right].$$ Plugging in $\Gamma' = \frac{\eps^2\cdot L}{16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell}$, we finally have $$\Pr\bigg[\big|\delta(y') - \mathbb{M} \, \delta \big| > \frac{\eps \cdot L}{2} \bigg] \le \exp\left[\frac{-\eps^2\cdot L^2}{16 \cdot \rho^2 \cdot L \cdot \Gamma'}\right] = \frac{1}{2n},$$
    thus completing the proof.
\end{proof}
   
\begin{proof} [Proof of \cref{thm:highway-demands}]
    \Cref{alg:demand_alg} probes all the hidden variable in the set: $\{y_i: \Omega_i > \Gamma'\}$, where $\Gamma' = \frac{\eps^2\cdot L}{16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell}$. The total number of probes is the number of $\Gamma'$-effectively large clusters that intersect with the $\rho^\beta \cdot L$-radius ball. By applying \cref{lem:cluster_bounded} with $\Gamma = \Gamma'$ and $R = \rho^{\beta} \cdot L$, the number of probes is bounded by
    \begin{align*}
        h^2\cdot \left(\frac{\rho^\beta \cdot L}{\Gamma'}\right)^{\log h} &= h^2\cdot \left(\frac{\rho^\beta \cdot L \cdot  16\cdot \log 2n\cdot \rho^{3\beta} \cdot \ell}{\eps^2\cdot L}\right)^{\log h}\\
        &= h^2\cdot \left(\frac{16\cdot \log 2n\cdot \rho^{4\beta} \cdot \ell}{\eps^2}\right)^{\log h}\\
        &= \left(\frac{\log n\cdot \rho^{\beta} \cdot \ell}{\eps^2}\right)^{O(\log h)}.
    \end{align*}
    The real shortest path length is $\delta(y)$ and \cref{alg:demand_alg} returns the path with length $\hat{\delta} = \delta(y')$. We can view the real amount of unprobed demands as another sample from the distribution of unprobed demands. By applying the \cref{lem:concentrate} twice and union bound, we have 
    \begin{equation*}
        \Pr\big[ \big| \hat{\delta} - \delta(y)\big| > \eps \cdot L \big] \le \Pr\bigg[\big|\delta(y') - \mathbb{M} \, \delta \big| > \frac{\eps \cdot L}{2} \bigg] + \Pr\bigg[\big|\delta(y) - \mathbb{M} \, \delta \big| > \frac{\eps \cdot L}{2} \bigg] \le 1/n.
    \end{equation*}
    Therefore, \cref{alg:demand_alg} outputs a $(1+\eps)$-approximate shortest path in $G'$ with high probability, completing the proof. 
\end{proof}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

%%%%%%%%%%%%%%%%%%%
\newcommand{\cdd}{{\alpha}} % Doubling Dimension Notation
%%%%%%%%%%%%%%%%%%%
   

